EgoVLPv2: Egocentric Video-Language Pre-training with Fusion in the Backbone

Video-language pre-training (VLP) has become increasingly important due to its ability to generalize to various vision and language tasks. However, existing egocentric VLP frameworks utilize separate video and language encoders and learn task-specific cross-modal information only during fine-tuning, limiting the development of a unified system. In this work, we introduce the second generation of egocentric video-language pre-training (EgoVLPv2), a significant improvement from the previous generation, by incorporating cross-modal fusion directly into the video and language backbones. EgoVLPv2 learns strong video-text representation during pre-training and reuses the cross-modal attention modules to support different downstream tasks in a flexible and efficient manner, reducing fine-tuning costs. Moreover, our proposed fusion in the backbone strategy is more lightweight and compute-efficient than stacking additional fusion-specific layers. Extensive experiments on a wide range of VL tasks demonstrate the effectiveness of EgoVLPv2 by achieving consistent state-of-the-art performance over strong baselines across all downstream. Our project page can be found at https://shramanpramanick.github.io/EgoVLPv2/.

==> unused_tables_figures.tex <==
\begin{table}[!t]
\centering

\small
\setlength{\tabcolsep}{4pt}
\resizebox{0.99\columnwidth}{!}{\begin{tabular}{@{}l |c  c | c c | c c c c @{}}
\toprule

\multirow{3}{*}{\bf Method} & \multicolumn{2}{c |}{\bf Pre-training} & \multicolumn{2}{c |}{\bf EgoMCQ} & \multicolumn{4}{c}{\bf EgoNLQ validation set} \\ 

\cmidrule{2-9}

& \multirow{2}{*}{\# Data} & \multirow{2}{*}{Batch Size} & \multicolumn{2}{c |}{Accuracy (\%)} & \multicolumn{2}{c}{mIOU@0.3} & \multicolumn{2}{c}{mIOU@0.5} \\ 

& & & Intra & Inter & R@1 & R@5 & R@1 & R@5 \\

\midrule

SlowFast \cite{feichtenhofer2019slowfast} & $-$ & $-$ & $-$ & $-$ & 5.45 & 10.74 & 3.12 & 6.63 \\
EgoVLP \cite{linegocentric} & 3.8 M & 512 & 90.6 & 57.2 & 10.84 & 18.84 & 6.81 & 13.45 \\
\rowcolor{Light}
Ours & 3.8 M & 256 & & & & & & \\
\rowcolor{Light}
Ours & 3.8 M & 512 & & & & & & \\

\midrule

EgoVLP$^{\dagger} \cite{linegocentric} $ & 3.8 M & 1024 & \\
LAVILA \cite{zhao2022learning} & & 1024 & 93.8 & 59.9 & 10.53 & 19.13 & 6.69 & 13.68\\
\rowcolor{Light}
Ours & 3.8 M & 1024 & & & & & & \\

%\midrule
%EgoVLP$^{\dagger}$ & 2048 & \\
%\rowcolor{Light}
%Ours & 2048 & & & & & & \\

\midrule
\end{tabular}}
\caption{\textbf{Performance on EgoMCQ and EgoNLQ's validation set.} EgoVLP$^{\dagger}$ refers to our re-implementation with specified batch size. }\label{tab:egomcq_nlq}
%\vspace{-4mm}
\end{table}



\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.4\textwidth]{ICCV_Format/Figures/Results_Summary.pdf}
    \caption{\textbf{\textbf{\model} outperforms EgoVLP} across a number of egocentric video understanding tasks (cf. Table \ref{tab:downstream_tasks} for details), by learning a video-language representation using cross-modal attention fusion in the transformer backbone.}
    \label{fig:results_summary}
\end{figure}





\begin{table}[!t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\resizebox{0.50\textwidth}{!}{\begin{tabular}{@{}l | c c c | c c c | c c c | c c c | c c c @{}}
\toprule
\multirow{2}{*}{\bf Method} & \multicolumn{3}{c |}{\bf Video-$1$} & \multicolumn{3}{c |}{\bf Video-$2$} & \multicolumn{3}{c |}{\bf Video-$3$} & \multicolumn{3}{c |}{\bf Video-$4$} & \multicolumn{3}{c}{\bf Average} \\ 

%\cmidrule{2-16}

& P & R & F-$1$ & P & R & F-$1$ & P & R & F-$1$ & P & R & F-$1$ & P & R & F-$1$ \\ 

\midrule
SeqDPP \cite{gong2014diverse} & 53.43 & 29.81 & 36.59 & 44.05 & 46.65 & 43.67 & 49.25 & 17.44 & 25.26 & 11.14 & \bf 63.49 & 18.15 & 39.47 & 39.35 & 30.92 \\
SH-DPP \cite{sharghi2016query} & 50.56 & 29.64 & 35.67 & 42.13 & 46.81 & 42.72 & 51.92 & 29.24 & 36.51 & 11.51 & 62.88 & 18.62 & 39.03 & 42.14 & 33.38 \\
QC-DPP \cite{sharghi2017query} & 49.86 & \bf 53.38 & 48.68 & 33.71 & \underline{62.09} & 41.66 & 55.16 & 29.24 & 36.51 & 21.39 & \underline{63.12} & 29.96 & 40.03 & \bf 60.25 & 44.19 \\
TPAN \cite{zhang2018query} & 49.66 & 50.91 & 48.74 & 43.02 & 48.73 & 45.30 & 58.73 & 56.49 & 56.51 & \underline{36.70} & 35.96 & 33.64 & 47.03 & 48.02 & 46.05 \\
CHAN \cite{xiao2020convolutional} & 54.73 & 46.57 & 49.14 & 45.92 & 50.26 & 46.53 & 59.75 & \bf 64.53 & 58.65 & 25.23 & 51.16 & 33.42 & 46.40 & 53.13 & 46.94 \\
HVN \cite{jiang2019hierarchical} & 52.55 & \underline{52.91} & \underline{51.45} & 38.66 & \bf 62.70 & 47.49 & 60.28 & \underline{62.58} & 61.08 & 26.27 & 54.21 & 35.47 & 44.57 & \underline{58.10} & 48.87 \\
QSAN \cite{xiao2020query} & 48.41 & 52.34 & 48.52 & 46.51 & 51.36 & 46.64 & 56.78 & 61.14 & 56.93 & 30.54 & 46.90 & 34.25 & 45.56 & 52.94 & 46.59 \\
WHM \cite{nalla2020watch} & 54.58 & 52.51 & 50.96 & 48.12 & 52.15 & 48.28 & 58.48 & 61.66 & 58.41 & \bf 37.40 & 43.90 & \underline{39.18} & 49.64 & 52.55 & 49.20 \\
IntentVizor \cite{wu2022intentvizor} & \underline{62.19} & 45.23 & 51.27 & 50.43 & 57.81 & 53.48 & \underline{73.45} & 53.56 & \underline{61.58} & 28.24 & 56.47 & 37.25 & \underline{53.58} & 53.27 & \underline{50.90} \\
\midrule
EgoVLP$^{\dagger}$ \cite{linegocentric} & 61.05 & 44.09 & 50.09 & \underline{51.27} & 58.77 & \underline{54.36} & 71.40 & 52.44 & 60.15 & 28.19 & 56.43 & 37.20 & 52.97 & 52.93 & 50.45 \\
\rowcolor{Light}
\model\ & \bf 66.47 & 46.86 & \bf 54.97 & \bf 51.89 & 60.20 & \bf 55.74 & \bf 76.35 & 55.24 & \bf 64.10 & 30.87 & 60.28 & \bf 40.83 & \bf 56.40 & 55.65 & \bf 53.91\\

\midrule

\bf \textcolor{blue}{$\Delta_{\text{Ours - EgoVLP}}$} & \textcolor{blue}{5.42} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{2.77} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{4.88} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{0.62} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{1.43} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{1.38} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{4.95} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{2.80} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{3.95} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{2.68} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{3.85} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{3.63} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{3.43} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{2.72} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{3.46} \textcolor{blue}{$\uparrow$}\\

\bottomrule
\end{tabular}}
\captionof{table}{\textbf{Performance on query-focused video summarization (QFVS).} Existing baselines are trained end-to-end, whereas \model\ only learns a tiny head on top of pre-trained encoders. $^{\dagger}$EgoVLP denotes the performance achieved by the officially released checkpoint.  }\label{tab:main_qfvs}

\end{table}



\begin{figure*}
     \centering
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ICCV_Format/Figures/Categories/dual.png}
         \caption{Dual Encoders}
         \label{fig:dual}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ICCV_Format/Figures/Categories/merged.png}
         % \vspace{-2em}
         \caption{Encoders w/ Stacked Fusion Layers}
         \label{fig:stacked}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ICCV_Format/Figures/Categories/shared.png}
         \caption{Shared Encoders}
         \label{fig:shared}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ICCV_Format/Figures/Categories/fused.png}
         \caption{Fusion in the Backbone (Ours)}
         \label{fig:fused}
     \end{subfigure}
        \vspace{-2mm}
    \caption{\textbf{Four different categories of video-language pre-training frameworks.} 
    (a) Dual Encoders: separate video and text backbones, InfoNCE~\cite{oord2018representation} as  common pretraining objective.
    (b) Encoders with Stacked Fusion Layers: \cite{} Cross-modal fusion layers on top of dual enc.
    (c) Shared Encoders: \cite{} One
     encoder for
      different modalities. Common pretraining task: MLM, VTM.
    (d) Fusion in the Backbone (Ours): }
    \label{fig:system_categories}
\end{figure*}


\begin{table}[!t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\resizebox{0.75\columnwidth}{!}{\begin{tabular}{@{} l | c c c c c c @{}}

\toprule

\multirow{2}{*}{\bf Cross-Att} & \multicolumn{6}{c}{\textbf{Learned value of $\alpha$}}  \\ 

& L7 & L8 & L9 & L10 & L11 & L12 \\

\midrule

Video-to-Text & \\
Text-to-video & \\

\bottomrule
\end{tabular}}
\caption{\textbf{}}
\label{tab:albation_supp_alpha_values}
\vspace{-2mm}
\end{table}

% \begin{table}[!t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \resizebox{0.4\columnwidth}{!}{\begin{tabular}{@{} c | c c @{}}

% \toprule

% \multirow{2}{*}{\bf Batch Size} & \multicolumn{2}{c}{\textbf{EgoMCQ} (\%)}  \\ 

% & Inter & Intra \\

% \midrule
% 128 & 90.6 & 59.8\\
% \rowcolor{Light}
% 256 & \bf 91.0 & \bf 60.9 \\
% 512 & \bf91.0 & 60.6\\
% 1024 & 90.8 & 60.5\\


% \bottomrule
% \end{tabular}}
% \caption{\textbf{}}
% \label{tab:albation_supp_batchsize}
% \vspace{-2mm}
% \end{table}


% \begin{table}[!t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \resizebox{0.4\columnwidth}{!}{\begin{tabular}{@{} c | c c @{}}

% \toprule

% \multirow{2}{1.9cm}{\bf \centering \# Frames (Pre-training)} & \multicolumn{2}{c}{\textbf{EgoMCQ} (\%)}  \\ 

% & Inter & Intra \\

% \midrule
% 2 & 90.1 & 56.7\\
% \rowcolor{Light}
% 4 & 91.0 & 60.9 \\
% 5 & 91.2 & 61.0\\
% 6 & 91.4 & 61.3\\


% \bottomrule
% \end{tabular}}
% \caption{\textbf{}}
% \label{tab:albation_supp_batchsize}
% \vspace{-2mm}
% \end{table}

%----------------------------------
%% SUBTABLE

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.9\textwidth]{ICCV_Format/Figures/Supplementary_Figs/QFVS_pipeline.pdf}
    \caption{QFVS Pipeline}
    \label{fig:qfvs_pipeline}
\end{figure*}

\vspace{1mm}

\noindent \textbf{EgoTaskQA:}

\vspace{1mm}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.95\textwidth]{ICCV_Format/Figures/Supplementary_Figs/QFVS_visualization_highres_compressed.png}
    \caption{QFVS.}
    \label{fig:qfvs}
\end{figure*}

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ICCV_Format/Figures/Supplementary_Figs/EgoMCQ_retrieval_visualizations_intra_compressed.png}
         \caption{Intra}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ICCV_Format/Figures/Supplementary_Figs/EgoMCQ_retrieval_visualizations_inter_compressed.png}
         \caption{Inter}
     \end{subfigure}
    % \vspace{-.5mm}
         \caption{EgoMCQ}
    % \vspace{-1.5mm}
    \label{fig:egomcq}
\end{figure*}
